Efficient Task Grouping Through Samplewise Optimisation Landscape Analysis

Shared training approaches, such as multi-task learning (MTL) and gradient-based meta-learning, are widely used in various machine learning applications, but they often suffer from negative transfer, leading to performance degradation in specific tasks. While several optimisation techniques have been developed to mitigate this issue for pre-selected task cohorts, identifying optimal task combinations for joint learning - known as task grouping - remains underexplored and computationally challenging due to the exponential growth in task combinations and the need for extensive training and evaluation cycles. This paper introduces an efficient task grouping framework designed to reduce these overwhelming computational demands of the existing methods. The proposed framework infers pairwise task similarities through a sample-wise optimisation landscape analysis, eliminating the need for the shared model training required to infer task similarities in existing methods. With task similarities acquired, a graph-based clustering algorithm is employed to pinpoint near-optimal task groups, providing an approximate yet efficient and effective solution to the originally NP-hard problem. Empirical assessments conducted on 8 different datasets highlight the effectiveness of the proposed framework, revealing a five-fold speed enhancement compared to previous state-of-the-art methods. Moreover, the framework consistently demonstrates comparable performance, confirming its remarkable efficiency and effectiveness in task grouping.

==> tables/ablation_study.tex <==
\begin{table*}[ht!]
\caption{The ablation study on video \protect\say{V04} of EasyCom-Clustering with known cluster number. The baseline model in the first row is a transformer trained with the paradigm in Fig. \ref{fig: idea_explain} (\textit{Middle}), i.e. a CT TRSF.
The option \protect\say{a} in each component is considered as the naive solution and are gradually replaced by others to illustrate the improvement.}
\centering
\scriptsize
\begin{tabularx}{0.86\linewidth}{viiiyiiiii}
\toprule
  & \multicolumn{2}{c}{\textbf{Temporal Aug.} $\op{\tau}$} & \multicolumn{3}{c}{\textbf{Centre Representation}} & \multicolumn{2}{c}{\textbf{Centre Learning Rate $\eta$}} &
  \multicolumn{2}{c}{\textbf{EasyCom-Clustering}} \\
 & \multicolumn{1}{c}{a} & \multicolumn{1}{c}{b} & \multicolumn{1}{c}{a} & \multicolumn{1}{c}{b} & \multicolumn{1}{c}{c} & \multicolumn{1}{c}{a} & \multicolumn{1}{c}{b} & \multicolumn{2}{c}{V04} \\
\multirow{-3}{*}{\textbf{\shortstack{Video \\Centres}}} & Uniform & Consect. & Last Forw. & Alg. \ref{alg:optimise} Incomp. & Alg. \ref{alg:optimise} & Incremental & Proportional & NMI (\%) & WCP (\%) \\
\cmidrule(l{4pt}r{0pt}){1-1} 
\cmidrule(l{10pt}r{10pt}){2-3} 
\cmidrule(l{7pt}r{12pt}){4-6}
\cmidrule(l{8pt}r{0pt}){7-8}
\cmidrule(l{8pt}r{8pt}){9-10} 
- & - & - & - & - & - & - & - & 85.20 & 95.19 \\
\checkmark & \checkmark & - & \checkmark & - & - & \checkmark & - & 83.54 & 93.89 \\
\checkmark & - & \checkmark & \checkmark & - & - & \checkmark & - & 83.97 & 94.31 \\
\checkmark & - & \checkmark & - & \checkmark & - & \checkmark & - & 86.20 & 95.94 \\
\checkmark & - & \checkmark & - & - & \checkmark & \checkmark & - & 87.19 & 96.30 \\
\checkmark & - & \checkmark & - & - & \checkmark & - & \checkmark & \textbf{90.69} & \textbf{97.83} \\
\bottomrule
\end{tabularx}
\label{tab: ablation} 
\end{table*}

==> tables/ablation_study_pe.tex <==
\begin{table}[ht!]
\caption{The ablation study of different Positional Embedding (PE) options on \protect\say{V08} of EasyCom-Clustering dataset (known cluster).}
\centering
\scriptsize
\begin{tabularx}{0.98\linewidth}{kkjj}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\shortstack{\textbf{Positional} \\ \textbf{Embedding}}} & \multicolumn{2}{c}{V08} \\
 &  & NMI (\%) & WCP (\%) \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-4}  
Temp. AVG \cite{Sharma2017ASimple} & \multirow{5}{*}{-} & 61.89 & 70.88 \\
SSiam \cite{sharma2019self} &  & 74.79 & 88.99 \\
CCL \cite{sharma2020clustering} &  & 83.99 & 93.98 \\
TSiam \cite{sharma2019self} &  & 82.17 & 92.61 \\
CT TRSF. &  & 82.57 & 94.05 \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-4}
\multirow{3}{*}{VC TRSF. (Ours)} & No PE & \textbf{86.70} & 95.10 \\
 & Scaled PE \cite{li2019neural} & 84.53 & 95.28 \\
 & Interpolated PE \cite{bertasius2021space} & 85.89 & \textbf{95.33}  \\
\bottomrule
\end{tabularx}
\label{tab: pe_ablation} 
\end{table}

==> tables/bbt_known.tex <==
\begin{table*}[ht!]
\caption{Video clustering performance of different methods on BBT dataset with known cluster numbers. The true cluster number of each video is post-appended to the video name.  }
\centering
\scriptsize
\begin{tabularx}{0.8\linewidth}{siiiiiiiiiiii}
\toprule
& \multicolumn{12}{c}{\textbf{BBT} (\%), Known Cluster Number} \\
\cmidrule(l{5pt}r{3pt}){2-13} 
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{s01e01 (8)} & \multicolumn{2}{c}{s01e02 (6)} & \multicolumn{2}{c}{s01e03 (26)} & \multicolumn{2}{c}{s01e04 (28)} & \multicolumn{2}{c}{s01e05 (25)} & \multicolumn{2}{c}{s01e06 (37)} \\
 & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP \\
   \cmidrule(l{16pt}r{16pt}){1-1} 
  \cmidrule(l{5pt}r{3pt}){2-3} 
  \cmidrule(l{5pt}r{3pt}){4-5}
  \cmidrule(l{5pt}r{3pt}){6-7}
  \cmidrule(l{5pt}r{3pt}){8-9}
  \cmidrule(l{5pt}r{3pt}){10-11}
  \cmidrule(l{5pt}r{3pt}){12-13} 
Temp. AVG \cite{Sharma2017ASimple} & 95.74 & 97.87 & 87.80 & 95.45 & 89.46 & 96.82 & 83.74 & 95.60 & 91.57 & 97.52 & 83.10 & 91.79 \\
SSiam \cite{sharma2019self} & 97.49 & 99.39 & 93.44 & 98.54 & 95.92 & 97.12 & 88.01 & 96.25 & 94.35 & 97.90 & 84.87 & 92.86 \\
CCL \cite{sharma2020clustering} & 98.06 & 98.63 & 96.27 & 99.51 & 95.30 & 97.27 & 91.03 & \textbf{97.06} & 96.78 & 97.71 & \textbf{86.45} & 92.50 \\
TSiam \cite{sharma2019self} & 97.06 & 98.48 & 95.46 & 99.51 & \textbf{96.91} & 97.12 & \textbf{91.55} & 96.08 & \textbf{97.40} & 98.28 & 86.30 & 92.74 \\
CT TRSF. & 97.51 & 99.09 & 97.32 & 99.19 & 93.01 & 96.52 & 86.70 & 95.92 & 92.63 & 98.09 & 84.02 & 91.79 \\
  \cmidrule(l{5pt}r{3pt}){2-3} 
  \cmidrule(l{5pt}r{3pt}){4-5}
  \cmidrule(l{5pt}r{3pt}){6-7}
  \cmidrule(l{5pt}r{3pt}){8-9}
  \cmidrule(l{5pt}r{3pt}){10-11}
  \cmidrule(l{5pt}r{3pt}){12-13} 
VC TRSF. (Ours) & \textbf{98.52} & \textbf{99.39} & \textbf{99.32} & \textbf{99.84} & 96.60 & \textbf{97.58} & 91.13 & 96.41 & 94.70 & \textbf{98.47} & 84.91 & \textbf{93.33} \\
\bottomrule
\end{tabularx}
\label{tab: bbt_known} 
\end{table*}

==> tables/bbt_unknown.tex <==
\begin{table*}[t!]
\caption{Video clustering performance of different methods on BBT dataset with unknown cluster numbers. The true cluster number of each video is post-appended to the video name. \protect\say{\#C} refers to the predicted cluster number. 
}
\centering
\scriptsize
\begin{tabularx}{0.7\linewidth}{svivivivivivi}
\toprule
& \multicolumn{12}{c}{\textbf{BBT} (\%), Unknown Cluster Number} \\
\cmidrule(l{5pt}r{3pt}){2-13} 
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c}{s01e01 (8)} & \multicolumn{2}{c}{s01e02 (6)} & \multicolumn{2}{c}{s01e03 (26)} & \multicolumn{2}{c}{s01e04 (28)} & \multicolumn{2}{c}{s01e05 (25)} & \multicolumn{2}{c}{s01e06 (37)} \\
 & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI \\
 \cmidrule(l{16pt}r{16pt}){1-1} 
   \cmidrule(l{5pt}r{3pt}){2-3} 
  \cmidrule(l{5pt}r{3pt}){4-5}
  \cmidrule(l{5pt}r{3pt}){6-7}
  \cmidrule(l{5pt}r{3pt}){8-9}
  \cmidrule(l{5pt}r{3pt}){10-11}
  \cmidrule(l{5pt}r{3pt}){12-13} 
Temp. AVG \cite{Sharma2017ASimple} & 7 & 95.43 & 8 & 89.80 & 11 & 91.01 & 13 & 87.80 & 11 & \textbf{94.45} & 22 & 83.07 \\
SSiam \cite{sharma2019self} & \textbf{7} & 87.05 & 6 & 89.44 & 16 & 90.20 & 10 & 85.58 & 8 & 89.12 & 9 & 71.37 \\
CCL \cite{sharma2020clustering} & 6 & 96.45 & 5 & 98.55 & 13 & 93.54 & 12 & 89.60 & 7 & 89.15 & 12 & 79.53 \\
TSiam \cite{sharma2019self} & 6 & 95.59 & 5 & 98.55 & \textbf{18} & \textbf{95.24} & \textbf{14} & 90.83 & \textbf{14} & 93.66 & 12 & 82.62 \\
CT TRSF. & 5 & 94.80 & \textbf{6} & 97.32 & 11 & 90.81 & 11 & 88.84 & 9 & 89.25 & 12 & 79.20 \\
   \cmidrule(l{5pt}r{3pt}){2-3} 
  \cmidrule(l{5pt}r{3pt}){4-5}
  \cmidrule(l{5pt}r{3pt}){6-7}
  \cmidrule(l{5pt}r{3pt}){8-9}
  \cmidrule(l{5pt}r{3pt}){10-11}
  \cmidrule(l{5pt}r{3pt}){12-13} 
VC TRSF. (Ours) & 6 & \textbf{97.06} & 5 & \textbf{98.81} & 12 & 94.11 & 11 & \textbf{91.03} & 11 & 92.50 & \textbf{29} & \textbf{84.17} \\
\bottomrule
\end{tabularx}
\label{tab: bbt_unknown} 
\end{table*}

==> tables/easycom_known.tex <==
\begin{table*}[ht]
\caption{Video clustering performance of different methods on EasyCom-Clustering dataset with known cluster numbers. The true cluster number of each video is post-appended to the video name. }
\centering
\scriptsize
\begin{tabularx}{0.99\linewidth}{siiiiiiiiiiiiiiiiiiiiii}
\toprule
 & \multicolumn{22}{c}{\textbf{EasyCom-Clustering} (\%), Known Cluster Number} \\
 \cmidrule(l{5pt}){2-23} 
 & \multicolumn{2}{c}{V01 (4)} & \multicolumn{2}{c}{V02 (3)} & \multicolumn{2}{c}{V03 (3)} & \multicolumn{2}{c}{V04 (3)} & \multicolumn{2}{c}{V05 (4)} & \multicolumn{2}{c}{V06 (3)} & \multicolumn{2}{c}{V07 (3)} & \multicolumn{2}{c}{V08 (4)} & \multicolumn{2}{c}{V09 (3)} & \multicolumn{2}{c}{V10 (3)} & \multicolumn{2}{c}{V11 (3)} \\
\multirow{-2}{*}{\textbf{Methods}} & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP \\
\cmidrule(l{3pt}r{3pt}){1-1} 
 \cmidrule(l{7pt}r{0pt}){2-3}  \cmidrule(l{7pt}r{0pt}){4-5}  \cmidrule(l{7pt}r{0pt}){6-7}
  \cmidrule(l{7pt}r{0pt}){8-9}
   \cmidrule(l{7pt}r{0pt}){10-11}
    \cmidrule(l{7pt}r{0pt}){12-13}
    \cmidrule(l{7pt}r{0pt}){14-15}
    \cmidrule(l{7pt}r{0pt}){16-17}
    \cmidrule(l{7pt}r{0pt}){18-19}
    \cmidrule(l{7pt}r{0pt}){20-21}
    \cmidrule(l{7pt}r{0pt}){22-23}
Temp. AVG \cite{Sharma2017ASimple} & 85.96 & 91.44 & 45.99 & 58.37 & 80.36 & 94.00 & 75.31 & 92.34 & 53.63 & 53.63 & 37.56 & 54.10 & 81.04 & 94.80 & 61.89 & 70.88 & 69.88 & 91.63 & 61.36 & 87.27 & 55.83 & 79.48 \\
SSiam \cite{sharma2019self} & 90.93 & 96.96 & 79.06 & 94.18 & 91.19 & 98.26 & 79.76 & 94.49 & 80.94 & 92.84 & 73.66 & 90.01 & 91.07 & 98.26 & 74.79 & 88.99 & 79.31 & 92.52 & 82.87 & 94.73 & 81.89 & 95.07 \\
CCL \cite{sharma2020clustering} & 94.39 & 98.45 & 80.11 & 94.47 & 92.79 & 98.52 & 83.93 & 94.36 & 89.49 & \textbf{97.41} & 76.73 & 92.13 & 92.07 & 98.39 & 83.99 & 93.98 & 89.38 & 97.07 & 75.67 & 93.20 & 79.47 & 94.18 \\
TSiam \cite{sharma2019self} & 95.25 & 98.79 & 79.69 & 93.53 & 87.65 & 96.60 & 84.44 & 95.03 & \textbf{90.66} & 97.01 & 78.29 & 91.96 & 90.79 & 98.09 & 82.17 & 92.61 & 74.80 & 91.69 & 83.17 & 94.05 & 84.62 & 95.35 \\
CT TRSF. & 90.16 & 95.33 & 74.41 & 91.87 & 94.40 & 98.88 & 85.20 & 95.19 & 80.09 & 91.10 & 76.46 & 92.21 & 91.54 & 98.05 & 82.57 & 94.05 & 85.99 & 94.79 & 81.29 & 91.89 & 80.37 & 93.82 \\
\cmidrule(l{7pt}r{0pt}){2-3}  \cmidrule(l{7pt}r{0pt}){4-5}  \cmidrule(l{7pt}r{0pt}){6-7}
  \cmidrule(l{7pt}r{0pt}){8-9}
   \cmidrule(l{7pt}r{0pt}){10-11}
    \cmidrule(l{7pt}r{0pt}){12-13}
    \cmidrule(l{7pt}r{0pt}){14-15}
    \cmidrule(l{7pt}r{0pt}){16-17}
    \cmidrule(l{7pt}r{0pt}){18-19}
    \cmidrule(l{7pt}r{0pt}){20-21}
    \cmidrule(l{7pt}r{0pt}){22-23}
VC TRSF. (Ours) & \textbf{96.26} & \textbf{99.02} & \textbf{82.25} & \textbf{95.35} & \textbf{94.86} & \textbf{99.05} & \textbf{90.69} & \textbf{97.83} & 87.39 & 96.01 & \textbf{79.81} & \textbf{92.43} & \textbf{93.29} & \textbf{98.59} & \textbf{86.70} & \textbf{95.10} & \textbf{98.17} & \textbf{99.75} & \textbf{89.47} & \textbf{97.52} & \textbf{87.12} & \textbf{95.70} \\
 \midrule \midrule  
 & \multicolumn{2}{c}{V12 (3)} & \multicolumn{2}{c}{V13 (3)} & \multicolumn{2}{c}{V14 (5)} & \multicolumn{2}{c}{V15 (3)} & \multicolumn{2}{c}{V16 (3)} & \multicolumn{2}{c}{V17 (3)} & \multicolumn{2}{c}{V18 (3)} & \multicolumn{2}{c}{V19 (3)} & \multicolumn{2}{c}{V20 (3)} & \multicolumn{2}{c}{V21 (5)} & \multicolumn{2}{c}{V22 (4)} \\
& NMI & WCP  & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP & NMI & WCP \\
 \cmidrule(l{7pt}r{0pt}){2-3}  \cmidrule(l{7pt}r{0pt}){4-5}  \cmidrule(l{7pt}r{0pt}){6-7}
  \cmidrule(l{7pt}r{0pt}){8-9}
   \cmidrule(l{7pt}r{0pt}){10-11}
    \cmidrule(l{7pt}r{0pt}){12-13}
    \cmidrule(l{7pt}r{0pt}){14-15}
    \cmidrule(l{7pt}r{0pt}){16-17}
    \cmidrule(l{7pt}r{0pt}){18-19}
    \cmidrule(l{7pt}r{0pt}){20-21}
    \cmidrule(l{7pt}r{0pt}){22-23}
Temp. AVG \cite{Sharma2017ASimple} & 66.59 & 88.63 & 39.30 & 71.07 & 82.68 & 85.43 & 38.24 & 58.15 & 91.32 & 98.11 & 62.60 & 61.86 & 82.40 & 93.91 & 59.95 & 64.59 & 77.97 & 92.92 & 60.23 & 66.50 & 60.90 & 76.61 \\
SSiam \cite{sharma2019self} & 83.87 & 95.30 & 88.85 & 97.30 & 84.11 & 84.65 & 79.52 & 94.31 & 92.41 & 98.16 & 62.06 & 61.78 & 92.03 & 98.45 & 94.06 & 98.75 & 88.29 & 96.75 & 82.04 & 91.67 & 82.59 & 94.09 \\
CCL \cite{sharma2020clustering} & 86.63 & 96.84 & 88.71 & 97.03 & 89.25 & \textbf{96.25} & 86.85 & 96.94 & 95.45 & 99.10 & 61.12 & 61.86 & 89.38 & 97.45 & 93.86 & 98.66 & 89.46 & 97.80 & 85.36 & 93.49 & 84.44 & 94.01 \\
TSiam \cite{sharma2019self} & 86.85 & 96.56 & 85.36 & 95.67 & 89.34 & 95.59 & 89.49 & 97.32 & 94.84 & 98.90 & 91.00 & 97.72 & 90.87 & 97.81 & 97.62 & 99.58 & 89.61 & 97.70 & \textbf{85.88} & 93.07 & 83.82 & 93.77 \\
CT TRSF. & 81.08 & 93.62 & 87.76 & 96.76 & 89.89 & \textbf{96.25} & 83.99 & 95.23 & 83.60 & 95.03 & 73.13 & 85.65 & 90.68 & 97.90 & 93.41 & 98.43 & 90.97 & 98.07 & 80.42 & 91.65 & 81.20 & 93.07 \\
 \cmidrule(l{7pt}r{0pt}){2-3}  \cmidrule(l{7pt}r{0pt}){4-5}  \cmidrule(l{7pt}r{0pt}){6-7}
  \cmidrule(l{7pt}r{0pt}){8-9}
   \cmidrule(l{7pt}r{0pt}){10-11}
    \cmidrule(l{7pt}r{0pt}){12-13}
    \cmidrule(l{7pt}r{0pt}){14-15}
    \cmidrule(l{7pt}r{0pt}){16-17}
    \cmidrule(l{7pt}r{0pt}){18-19}
    \cmidrule(l{7pt}r{0pt}){20-21}
    \cmidrule(l{7pt}r{0pt}){22-23}
VC TRSF. (Ours) & \textbf{90.89} & \textbf{98.30} & \textbf{92.99} & \textbf{98.61} & \textbf{90.20} & 95.87 & \textbf{92.96} & \textbf{98.55} & \textbf{97.22} & \textbf{99.46} & \textbf{95.37} & \textbf{99.11} & \textbf{93.15} & \textbf{98.63} & \textbf{98.41} & \textbf{99.72} & \textbf{93.80} & \textbf{98.80} & 84.35 & \textbf{94.04} & \textbf{86.97} & \textbf{96.38} \\
\bottomrule
\end{tabularx}
\label{tab: easycom_known} 
\end{table*}

==> tables/easycom_unknown.tex <==
\begin{table*}[ht]
\caption{Video clustering performance of different methods on EasyCom-Clustering dataset with unknown cluster numbers. The true cluster number of each video is post-appended to the video name. \protect\say{\#C} refers to the predicted cluster number. } 
\centering
\scriptsize
\begin{tabularx}{0.99\linewidth}{svivivivivivivivivivivi}
\toprule
& \multicolumn{22}{c}{\textbf{EasyCom-Clustering} (\%), Unknown Cluster Number} \\
\cmidrule(l{5pt}){2-23} 
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c}{V01 (4)} & \multicolumn{2}{c}{V02 (3)} & \multicolumn{2}{c}{V03 (3)} & \multicolumn{2}{c}{V04 (3)} & \multicolumn{2}{c}{V05 (4)} & \multicolumn{2}{c}{V06 (3)} & \multicolumn{2}{c}{V07 (3)} & \multicolumn{2}{c}{V08 (4)} & \multicolumn{2}{c}{V09 (3)} & \multicolumn{2}{c}{V10 (3)} & \multicolumn{2}{c}{V11 (3)} \\
 & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI \\
 \cmidrule(l{9pt}r{9pt}){1-1} 
  \cmidrule(l{6pt}r{0pt}){2-3}  \cmidrule(l{6pt}r{0pt}){4-5}  \cmidrule(l{6pt}r{0pt}){6-7}
  \cmidrule(l{6pt}r{0pt}){8-9}
   \cmidrule(l{6pt}r{0pt}){10-11}
    \cmidrule(l{6pt}r{0pt}){12-13}
    \cmidrule(l{6pt}r{0pt}){14-15}
    \cmidrule(l{6pt}r{0pt}){16-17}
    \cmidrule(l{6pt}r{0pt}){18-19}
    \cmidrule(l{6pt}r{0pt}){20-21}
    \cmidrule(l{6pt}r{0pt}){22-23}
Temp. AVG \cite{Sharma2017ASimple} & 2 & 61.36 & 2 & 19.46 & 2 & 55.09 & 2 & 69.27 & 3 & 51.58 & 3 & 37.56 & 3 & 81.04 & \textbf{3} & 59.44 & 2 & 84.08 & 2 & 18.82 & 1 & 0.00 \\
SSiam \cite{sharma2019self} & 5 & 92.15 & 4 & 76.76 & 4 & 85.80 & 5 & 82.86 & 5 & 82.71 & 4 & 77.71 & 4 & 90.05 & 6 & \textbf{84.54} & 4 & 89.89 & 5 & 81.56 & 4 & 78.57 \\
CCL \cite{sharma2020clustering} & 7 & 90.05 & 9 & 71.92 & 7 & 86.21 & 4 & 83.16 & 10 & 84.37 & 7 & 74.60 & 5 & 88.21 & 9 & 84.53 & 5 & 91.92 & 6 & 78.33 & 7 & 78.73 \\
TSiam \cite{sharma2019self} & 7 & \textbf{92.31} & 7 & 80.12 & 7 & 85.09 & 7 & 82.16 & 8 & \textbf{86.34} & 7 & \textbf{84.04} & 7 & 88.17 & 7 & 83.86 & 5 & 86.06 & 6 & 83.11 & 6 & 81.09 \\
CT TRSF. & \textbf{4} & 90.16 & 3 & 74.41 & 3 & 94.40 & 3 & 85.2 & 5 & 82.37 & 2 & 33.74 & 3 & 91.54 & 6 & 79.45 & 3 & 85.99 & 4 & 70.40 & 3 & 80.37 \\
   \cmidrule(l{6pt}r{0pt}){2-3}  \cmidrule(l{6pt}r{0pt}){4-5}  \cmidrule(l{6pt}r{0pt}){6-7}
  \cmidrule(l{6pt}r{0pt}){8-9}
   \cmidrule(l{6pt}r{0pt}){10-11}
    \cmidrule(l{6pt}r{0pt}){12-13}
    \cmidrule(l{6pt}r{0pt}){14-15}
    \cmidrule(l{6pt}r{0pt}){16-17}
    \cmidrule(l{6pt}r{0pt}){18-19}
    \cmidrule(l{6pt}r{0pt}){20-21}
    \cmidrule(l{6pt}r{0pt}){22-23}
VC TRSF. (Ours) & 3 & 90.23 & \textbf{3} & \textbf{82.25} & \textbf{3} & \textbf{94.86} & \textbf{3} & \textbf{90.69} & \textbf{3} & 81.82 & \textbf{3} & 79.81 & \textbf{3} & \textbf{93.29} & 6 & 76.73 & \textbf{3} & \textbf{98.17} & \textbf{3} & \textbf{89.47} & \textbf{3} & \textbf{87.12} \\
 \midrule \midrule 
& \multicolumn{2}{c}{V12 (3)} & \multicolumn{2}{c}{V13 (3)} & \multicolumn{2}{c}{V14 (5)} & \multicolumn{2}{c}{V15 (3)} & \multicolumn{2}{c}{V16 (3)} & \multicolumn{2}{c}{V17 (3)} & \multicolumn{2}{c}{V18 (3)} & \multicolumn{2}{c}{V19 (3)} & \multicolumn{2}{c}{V20 (3)} & \multicolumn{2}{c}{V21 (5)} & \multicolumn{2}{c}{V22 (4)} \\
 & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI & \#C & NMI \\
   \cmidrule(l{6pt}r{0pt}){2-3}  \cmidrule(l{6pt}r{0pt}){4-5}  \cmidrule(l{6pt}r{0pt}){6-7}
  \cmidrule(l{6pt}r{0pt}){8-9}
   \cmidrule(l{6pt}r{0pt}){10-11}
    \cmidrule(l{6pt}r{0pt}){12-13}
    \cmidrule(l{6pt}r{0pt}){14-15}
    \cmidrule(l{6pt}r{0pt}){16-17}
    \cmidrule(l{6pt}r{0pt}){18-19}
    \cmidrule(l{6pt}r{0pt}){20-21}
    \cmidrule(l{6pt}r{0pt}){22-23}
Temp. AVG \cite{Sharma2017ASimple} & 2 & 48.56 & 3 & 39.30 & 2 & 52.23 & 1 & 0.00 & 2 & 46.91 & 2 & 49.97 & 2 & 46.79 & 2 & 65.42 & 3 & 77.97 & 2 & 34.74 & 3 & 59.21 \\
SSiam \cite{sharma2019self} & 4 & 82.46 & 6 & 86.50 & \textbf{7} & 83.37 & 3 & 79.52 & 3 & 92.41 & 3 & 62.06 & 5 & 90.18 & 3 & 94.06 & 4 & 88.08 & 8 & 81.82 & \textbf{5} & 82.60 \\
CCL \cite{sharma2020clustering} & 6 & 86.59 & 9 & 86.59 & 11 & 88.12 & 5 & 83.43 & 6 & 89.31 & 5 & 85.38 & 7 & 84.09 & 5 & 88.61 & 6 & 89.92 & 9 & 84.14 & 11 & 83.15 \\
TSiam \cite{sharma2019self} & 5 & 82.01 & 10 & 77.91 & 11 & \textbf{91.48} & 7 & \textbf{84.81} & 5 & 94.69 & 3 & \textbf{91.00} & 6 & 84.57 & 4 & 92.26 & 6 & 85.38 & 7 & \textbf{84.20} & 12 & \textbf{84.82} \\
CT TRSF. & 3 & 81.08 & 6 & 68.00 & 8 & 81.03 & \textbf{3} & 83.99 & 3 & 83.60 & \textbf{3} & 73.13 & 4 & 81.11 & 3 & 93.41 & \textbf{3} & \textbf{90.97} & \textbf{5} & 80.42 & 7 & 70.37 \\
   \cmidrule(l{6pt}r{0pt}){2-3}  \cmidrule(l{6pt}r{0pt}){4-5}  \cmidrule(l{6pt}r{0pt}){6-7}
  \cmidrule(l{6pt}r{0pt}){8-9}
   \cmidrule(l{6pt}r{0pt}){10-11}
    \cmidrule(l{6pt}r{0pt}){12-13}
    \cmidrule(l{6pt}r{0pt}){14-15}
    \cmidrule(l{6pt}r{0pt}){16-17}
    \cmidrule(l{6pt}r{0pt}){18-19}
    \cmidrule(l{6pt}r{0pt}){20-21}
    \cmidrule(l{6pt}r{0pt}){22-23}
VC TRSF. (Ours) & \textbf{3} & \textbf{90.89} & \textbf{3} & \textbf{92.99} & 8 & 84.50 & 2 & 72.89 & \textbf{3} & \textbf{97.22} & 4 & 86.23 & \textbf{3} & \textbf{93.15} & \textbf{3} & \textbf{98.41} & 4 & 89.05 & 7 & 79.57 & 7 & 74.27 \\
\bottomrule
\end{tabularx}
\label{tab: easycom_unknown} 
\end{table*}

==> tables/overall_performance.tex <==
\begin{table*}[t!]
\caption{The overall performance of different methods on BBT and EasyCom-Clustering with cluster number known/unknown. \protect\say{\#C DIF} refers to the sum of the absolute differences between the predicted and true cluster number of all videos of the dataset, which is the smaller the better. }
\centering
\scriptsize
\begin{tabularx}{0.8\linewidth}{kyyyyyyyy}
\toprule
 & \multicolumn{4}{c}{\textbf{BBT}} & \multicolumn{4}{c}{\textbf{EasyCom-Clustering}} \\
 \cmidrule(l{10pt}r{10pt}){2-5}  \cmidrule(l{10pt}r{10pt}){6-9} 
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{2}{c}{Known} & \multicolumn{2}{c}{Unknown} & \multicolumn{2}{c}{Known} & \multicolumn{2}{c}{Unknown} \\
& NMI (\%) & WCP (\%) & \#C DIF & NMI (\%) & NMI (\%) & WCP (\%) & \#C DIF & NMI (\%) \\
 \cmidrule(l{12pt}r{12pt}){1-1} 
 \cmidrule(l{8pt}r{8pt}){2-3} 
  \cmidrule(l{10pt}r{8pt}){4-5}
   \cmidrule(l{8pt}r{8pt}){6-7}
    \cmidrule(l{10pt}r{8pt}){8-9} 
Temp. AVG \cite{Sharma2017ASimple} & 88.57 & 95.84 & 62 & 90.26 & 65.05 & 78.44 & 25 & 48.13 \\
SSiam \cite{sharma2019self} & 92.34 & 97.01 & 74 & 85.46 & 83.42 & 93.07 & 27 & 83.89 \\
CCL \cite{sharma2020clustering} & 93.98 & 97.11 & 75 & 91.14 & 85.84 & 94.62 & 82 & 84.61 \\
TSiam \cite{sharma2019self} & 94.11 & 97.04 & 61 & 92.75 & 87.10 & 95.84 & 76 & 85.70 \\
CT TRSF. & 91.86 & 96.77 & 76 & 90.04 & 84.48 & 94.49 & 15 & 79.78 \\
 \cmidrule(l{8pt}r{8pt}){2-3} 
  \cmidrule(l{10pt}r{8pt}){4-5}
   \cmidrule(l{8pt}r{8pt}){6-7}
    \cmidrule(l{10pt}r{8pt}){8-9} 
VC TRSF. (Ours) & \textbf{94.20} & \textbf{97.50} & \textbf{56} & \textbf{92.95} & \textbf{91.01} & \textbf{97.45} & \textbf{15} & \textbf{87.44}  \\
\bottomrule
\end{tabularx}
\label{tab: overall_res} 
\end{table*}
